Combining Neural Networks and Tree Search for Task and Motion Planning in Challenging Environments

We consider task and motion planning in complex dynamic environments for problems expressed in terms of a set of Linear Temporal Logic (LTL) constraints, and a reward function. We propose a methodology based on reinforcement learning that employs deep neural networks to learn low-level control policies as well as task-level option policies. A major challenge in this setting, both for neural network approaches and classical planning, is the need to explore future worlds of a complex and interactive environment. To this end, we integrate Monte Carlo Tree Search with hierarchical neural net control policies trained on expressive LTL specifications. This paper investigates the ability of neural networks to learn both LTL constraints and control policies in order to generate task plans in complex environments. We demonstrate our approach in a simulated autonomous driving setting, where a vehicle must drive down a road in traffic, avoid collisions, and navigate an intersection, all while obeying given rules of the road.

==> related.tex <==
% TAMP
Task and Motion Planning (TAMP) approaches such as those proposed in \cite{toussaint2015logic,shivashankar2014towards} are powerful and efficient for solving spatial reasoning problems. 
One family of TAMP approaches for large state spaces involves the use of RRT-based planners to determine reachability and create efficient task plans~\cite{wolfe2010combined,shivashankar2014towards}. Such an approach requires concrete definitions both of subtasks and of goals associated with those tasks. It also does not necessarily lead to a solution that would be considered optimal by a human.
In contrast, Toussaint et al. proposed a TAMP algorithm based on optimizing a logical program~\cite{toussaint2015logic}. In practice, they hierarchically break the problem down into simpler sub-problems. Our work is similar in spirit in that it enables logical specification of desired (and undesired) behaviors using Linear Temporal Logic. %: the continuous action parametrization as well as their sequencing will be optimized to adhere to these specifications.

% OACs
These approaches suffer badly from the curse of dimensionality due to large state spaces and complex interactions with the environment.
One possible approach for avoiding this problem is given by \cite{wachter2013action} who describe the  Object-Action Complex (OAC) formalism.
OACs are the combination of a low-level controller, possibly one trained via reinforcement learning, and its associated preconditions and performance metrics. These preconditions translate to predicate conditions and effects that can be used with a PDDL planner. For example, \cite{ahmadzadeh2015learning} learn grounded motion primitives together with expected visual features.
Others such as \cite{kappler2015data} define a state machine together with a set of actions represented as Associative Skill Memories.
Similarly, others described a planning approach that searches through the tree of possible actions defined by a PDDL specification, where all individual actions were grounded through learning from demonstration~\cite{paxton2016want}.

% ------------------------------------------------------------------------------
% MCTS
%Rather than exhaustively searching through the massive tree of possible actions and reactions, we employ Monte Carlo Tree Search (MCTS).
%MCTS has previously been employed in complex, continuous domains through use of macro-actions, progressive un-pruning, and Continuous Rapid Action Value Estimates (cRAVE), but is not generally applied to robotics problems.
Sampling-based approaches for policy search are well suited to complex problems with multiple dynamic entities.
One widely used approach is Monte Carlo Tree Search (MCTS), which has been applied to high dimensional games and planning problems, including to solving Partially Observable MDPs (POMDPs) by~\cite{silver2010monte}.
%Jacobsen et al.~\cite{jacobsen2014monte} used macro actions, progressive widening, and roulette wheel selection in their MCTS planner applied to playing the game Mario, and Couetoux et al.~\cite{couetoux2011continuous} introduced cRAVE to deal with continuous state and action spaces.
%Our approach can be viewed through the lens of cRAVE and progressive widening as a way of associating explored state/actions with those that should be selected in order to perform approximately optimal action selection.
%\cite{couetoux2012improving} introduce Blind Values to help guide the search towards new decisions.
%In \cite{mansley2011sample}, the authors apply Hierarchal Optimistic Optimization to tree search, which is a sampling-based approach based on the HOO algorithm for $\mathcal{X}$-armed bandits by \cite{bubeck2009online}.
While originally developed for use with discrete sets of moves in a game, a number of modifications have been proposed that allow MCTS to be applied to continuous domains, including the work of \cite{mansley2011sample,couetoux2011continuous,couetoux2012improving,yee2016monte}.
Yee et al.~\cite{yee2016monte} propose Kernel Regression MCTS, which fits a kernel regression function to estimate value and number of visits to be used in tree search, in order to intelligently find additional values to expand.
Silver et al.~\cite{silver2016mastering} combined tree search and DRL to achieve master-level performance in go.
The MCTS facet of our approach is distinct from~\cite{couetoux2011continuous,yee2016monte} in that we explicitly distinguish between continuous parameterizations of an action and discrete action selection problems. In contrast to~\cite{silver2016mastering}, we are dealing with a continuous state space and LTL constraints instead of game-playing.
%We use prior information from expert demonstrations to initialize this search with ``good'' high-level discrete action distributions, although future work will examine alternate ways of initializing this data, e.g. from learning.

% ------------------------------------------------------------------------------
% SELF DRIVING CARS
In the self-driving vehicle domain, \cite{xu2016end} use a large video data set to jointly learn driving features, and \cite{bojarski2016end} use end to end learning to predict steering angle from video data.
Closest to our work, \cite{shalev2016safe} examine safe reinforcement learning for self driving cars. In particular, they note that rare penalties such as constraint violations need a proportionally larger weight. To deal with the variance due to corner cases, they decompose the policy $\pi$ into a mapping from $S$ to a set of ``desires'', and a mapping from the ``desires'' to an actual trajectory; the latter mapping is not learned, but rather implemented by solving an optimization problem with costs depending on the desires and hard constraints imposing functional safety. Like us, they also make use of the idea of options introduced by \cite{suttonPS99}, in order to to mitigate the effect of the task time horizon during learning.

% REINFORCEMENT LEARNING
In \cite{andreas2016modular}, the authors describe an algorithm for task level learning of options based on catalog learning with policy sketches. These sketches are a suggested sequence of options, which makes learning practical.
\cite{lample2016playing} used recurrent deep Q learning to train an agent to play the first person shooter Doom. They use a similar approach to our options, in that they train two different networks in different environments and combine them.

% LTL
One key challenge of RL methods is the requirement of an agent model that is Markovian. In this work, we augment the state space $S$ with memory, in the form of a deterministic Rabin automaton. This is similar to approaches in the formal methods literature like \cite{DingSBR14} which construct a product of an MDP and a Rabin automaton. However, in contrast with these approaches, we do not obtain an optimal MDP policy via dynamic programming, but approximate it via deep reinforcement learning.


